Dynamic Masking Rate Schedules for MLM Pretraining

Most works on transformers trained with the Masked Language Modeling (MLM) objective use the original BERT model's fixed masking rate of 15%. We propose to instead dynamically schedule the masking rate throughout training. We find that linearly decreasing the masking rate over the course of pretraining improves average GLUE accuracy by up to 0.46% and 0.25% in BERT-base and BERT-large, respectively, compared to fixed rate baselines. These gains come from exposure to both high and low masking rate regimes, providing benefits from both settings. Our results demonstrate that masking rate scheduling is a simple way to improve the quality of masked language models, achieving up to a 1.89x speedup in pretraining for BERT-base as well as a Pareto improvement for BERT-large.

==> conclusion.tex <==
\section{Conclusion}

We introduce the technique of scheduling the masking rate during MLM pretraining.
We demonstrate that linearly decreasing masking rate schedules improves downstream task performance for both \texttt{BERT-base} and \texttt{BERT-large}.
The quality improvement can also be used to reduce training time; linearly decreasing schedules achieve up to a 1.89x speedup in pretraining for \texttt{BERT-base} and are a Pareto improvement for \texttt{BERT-large}.

We also investigate the source of our method's success, demonstrating that dynamic scheduling matches the improved linguistic capabilities of a lower masking rate and the broad MLM performance of a higher masking rate.
We also show that a decreasing schedule is necessary for the success of dynamic masking rates.
% Finally, as scheduled masking outperforms constant masking at an increased rate but only masking according to a schedule without computing the loss on all masked tokens 
Finally, we demonstrate that neither the increased signal nor the masking pattern without the corresponding loss are alone sufficient to achieve the gains of masking rate scheduling.

Overall, our work shows that masking rate scheduling is a simple and reliable way to improve the quality and efficiency of MLM pretraining.

==> future-work.tex <==
\section{Future work}

\paragraph{Effective batch size.}
As noted in \ref{sec:ablations}, masking rate scheduling increases the number of tokens the loss is defined over.
One possible interpretation is that masking rate scheduling is effectively starting with a higher initial batch size and decreasing the batch size over the training duration.
Valuable further research would be to disambiguate the effect of scheduling the batch size on BERT pretraining.

\paragraph{Scheduling for encoder-decoder models.}
In this work we chose to evaluate the effect of masking rate scheduling on BERT which is an encoder only transformer.
Encoder-decoder transformer variants can also trained be using an MLM objective.
It would be interesting to determine whether the benefits of masking rate scheduling for BERT pretraining extend to encoder-decoder models as well.
Furthermore, it would be useful to determine how masking rate scheduling integrates with MLM variants such as span masking \cite{t5-raffel} or mixture of denoisers~\cite{ul2-tay}.

\paragraph{Broader evaluation of different scheduling techniques.}
This work introduces the concept of scheduled masking rates for MLM pretraining.
While we evaluate a broad group of schedulers and scheduler settings and demonstrate their downstream performance gains, future work could include the investigation of other scheduling techniques.
Such techniques could include warmup periods and cyclic rate scheduling \cite{cyclical-smith, warmup-goyal}.
